Learning to Discover Medicines

Discovering new medicines is the hallmark of human endeavor to live a better and longer life. Yet the pace of discovery has slowed down as we need to venture into more wildly unexplored biomedical space to find one that matches today's high standard. Modern AI-enabled by powerful computing, large biomedical databases, and breakthroughs in deep learning-offers a new hope to break this loop as AI is rapidly maturing, ready to make a huge impact in the area. In this paper we review recent advances in AI methodologies that aim to crack this challenge. We organize the vast and rapidly growing literature of AI for drug discovery into three relatively stable sub-areas: (a) representation learning over molecular sequences and geometric graphs; (b) data-driven reasoning where we predict molecular properties and their binding, optimize existing compounds, generate de novo molecules, and plan the synthesis of target molecules; and (c) knowledge-based reasoning where we discuss the construction and reasoning over biomedical knowledge graphs. We will also identify open challenges and chart possible research directions for the years to come.

==> pipeline.tex <==

\subsection{Drug discovery pipeline}

Drug discovery is the process to identify the new medicine. It involves
a wide range of scientific disciplines, including biology, chemistry
and pharmacology. The overall framework of drug development is rigours
and costly. There are four main stages going from drug discovery,
pre-clinical trial, clinical development, and finally pharmacovigilance.
\\

The drug discovery can be viewed as reasoning. The reasoning process
is to derive new knowledge from previous acquired knowledge in response
to a query. The drug discovery can be set up as query, database, answer
triplet. Then we can formulate different drug discovery related problem
using this triplet. For example the drug property classification,
the query is the toxicity of the drug, the database the structure
of the drug, and the answer is the toxicity of drug. Another example
is drug-target binding problem where drug is the query, target is
database, and the answer determining the binding between the drug
and protein.

Drug discovery is the process of learning to reason. (Try to elaborate
this idea) 

\subsection{Machine learning in drug discovery}

There are several direction we can go with the knowledge reasoning
but we can categorize it into three main direction. The first direction
is answering the question given the molecule, what is its properties.
Second, with the target protein in mind, what kind of molecule will
interact with it and wherever it is available through drug repurposing
or need to be generated from scratch. Finally, given a molecule, how
can we generate the molecule from the available materials, meaning
solving the synthetic tractability, reaction planning, or retrosynthesis
problem.

A powerful machine learning framework is the key of solving those
three questions. To solve those questions, a ML framework should has
expressiveness, learnability, and generalizability. Expressiveness
is in the sense that it can represent the complexity of biomedical
world. Learnability means that it can infer and combine the hidden
knowledge from the training data from one or many different domains.
Finally, generalizability is the ability to maintain the performance
with unseen data, which is the general case in discovering process.

